ANCHOR: A Port-Hamiltonian Model for Forecasting Team Dynamics in Human-in-the-Loop Systems

Cyber-physical-human systems close a loop around people by sensing human behavior, predict it and act on it. Human teams are a natural target, because collaboration breaks down in ways that a timely prompt could prevent. Collaborative mixed reality makes this loop practical, since each headset senses who speaks, where its wearer looks and who stands together, and it can deliver a light prompt. In this loop, the headsets are sensors, the prompts are actuators and the team is the plant. Closing the loop needs a plant model that is small enough to learn from few teams, safe to iterate and readable by a designer. We propose ANCHOR, which models a team as a ball in an energy bowl. The bottom of the bowl is where the team rests, and it is set by the team's recent behavior, its own history and other teams. Formally, ANCHOR is a switched port-Hamiltonian system with 52 parameters, and each part stands for a testable claim from team psychology. Because of this structure, for any fitted parameters, a forecast moves away from rest only when task progress or a prompt pushes it, and prompts of bounded size that are spaced in time move it a bounded distance. On \nGroups{} four-person teams held out from training, a team that drifts from its usual behavior returns most of the way within half a minute. After 32 s, about 24% of the deviation remains, and ANCHOR predicted 30%. Forecasts are clearly better when the resting point blends its three sources than when it uses one. ANCHOR matches the accuracy of a black-box baseline with about 40,000 parameters. It anticipates conversation collapse with an AUROC of 0.85. In simulation under assumed prompt effects, it removes 2.2 times as much breakdown time per prompt as periodic prompting.

==> tables/ablation.tex <==
Selected model & 52 & 0.758 & 1.082 & 1.002 \\
1st-order, diag & 45 & 0.762 & 1.088 & 1.011 \\
1st-order, diag, switched & 54 & 0.760 & 1.083 & 1.002 \\
1st-order, equiv & 69 & 0.769 & 1.093 & 1.013 \\
1st-order, equiv, switched & 95 & 0.771 & 1.086 & 0.998 \\
1st-order, full & 424 & 0.850 & 1.168 & 1.075 \\
1st-order, full, switched & 684 & 0.852 & 1.239 & 1.079 \\
2nd-order, diag & 52 & 0.759 & 1.086 & 1.009 \\
2nd-order, diag, switched & 61 & 0.761 & 1.088 & 1.016 \\
2nd-order, equiv & 76 & 0.763 & 1.088 & 1.011 \\
2nd-order, equiv, switched & 102 & 0.768 & 1.092 & 1.015 \\
2nd-order, full & 431 & 0.822 & 1.128 & 1.033 \\
2nd-order, full, switched & 691 & 0.864 & 1.175 & 1.062 \\
attractor: recent only & 40 & 0.887 & 1.293 & 1.152 \\
attractor: session only & 40 & 0.768 & 1.099 & 1.063 \\
no task-progress port & 47 & 0.771 & 1.123 & 1.057 \\
no friction features & 52 & 0.758 & 1.082 & 1.002 \\
no scale coupling & 53 & 0.759 & 1.082 & 1.001 \\
attractor only, no dynamics & 21 & 0.848 & 1.099 & 1.009 \\


==> tables/app_auroc.tex <==
\emph{Conversation collapse} & & & & & & \\
\quad ANCHOR (ours) & 0.80 & 0.83 & 0.78 & 0.80 & 0.76 & 0.78 \\
\quad Attractor only & 0.81 & 0.83 & 0.78 & 0.79 & 0.76 & 0.78 \\
\quad Persistence & 0.76 & 0.73 & 0.75 & 0.72 & 0.72 & 0.69 \\
\quad Recent average & 0.80 & 0.82 & 0.78 & 0.78 & 0.76 & 0.78 \\
\quad VAR(2) + aug. & 0.76 & 0.74 & 0.78 & 0.78 & 0.79 & 0.80 \\
\quad Ridge + aug. & 0.78 & 0.77 & 0.75 & 0.74 & 0.75 & 0.75 \\
\quad MLP + aug. & 0.75 & 0.74 & 0.74 & 0.74 & 0.74 & 0.74 \\
\emph{Loss of shared focus} & & & & & & \\
\quad ANCHOR (ours) & 0.81 & 0.75 & 0.74 & 0.70 & 0.67 & 0.62 \\
\quad Attractor only & 0.80 & 0.74 & 0.74 & 0.70 & 0.68 & 0.61 \\
\quad Persistence & 0.82 & 0.73 & 0.74 & 0.70 & 0.73 & 0.66 \\
\quad Recent average & 0.81 & 0.74 & 0.76 & 0.72 & 0.72 & 0.64 \\
\quad VAR(2) + aug. & 0.72 & 0.67 & 0.63 & 0.59 & 0.59 & 0.55 \\
\quad Ridge + aug. & 0.73 & 0.68 & 0.72 & 0.68 & 0.68 & 0.59 \\
\quad MLP + aug. & 0.75 & 0.69 & 0.71 & 0.65 & 0.66 & 0.58 \\
\emph{Spatial fragmentation} & & & & & & \\
\quad ANCHOR (ours) & 0.71 & 0.67 & 0.61 & 0.63 & 0.58 & 0.61 \\
\quad Attractor only & 0.71 & 0.64 & 0.61 & 0.60 & 0.57 & 0.58 \\
\quad Persistence & 0.74 & 0.68 & 0.62 & 0.65 & 0.57 & 0.59 \\
\quad Recent average & 0.71 & 0.64 & 0.61 & 0.60 & 0.57 & 0.59 \\
\quad VAR(2) + aug. & 0.69 & 0.66 & 0.54 & 0.55 & 0.44 & 0.42 \\
\quad Ridge + aug. & 0.72 & 0.66 & 0.68 & 0.70 & 0.65 & 0.66 \\
\quad MLP + aug. & 0.67 & 0.60 & 0.60 & 0.58 & 0.59 & 0.58 \\


==> tables/app_intervention.tex <==
Balance & ANCHOR & 0.25 & 13.3 & 12.4 / 0.18 & 12.3 / 0.24 & 12.0 / 0.23 & 12.8 / 0.34 \\
Balance & ANCHOR & 0.50 & 13.3 & 11.4 / 0.38 & 11.4 / 0.47 & 10.8 / 0.47 & 12.1 / 0.62 \\
Balance & ANCHOR & 1.00 & 13.3 & 9.9 / 0.68 & 9.8 / 0.94 & 8.9 / 0.93 & 9.8 / 1.06 \\
Attention & ANCHOR & 0.25 & 11.5 & 8.2 / 0.65 & 7.5 / 1.37 & 7.2 / 1.62 & 7.2 / 1.64 \\
Attention & ANCHOR & 0.50 & 11.5 & 5.7 / 1.15 & 5.6 / 2.41 & 5.3 / 2.98 & 5.6 / 3.22 \\
Attention & ANCHOR & 1.00 & 11.5 & 3.1 / 1.68 & 4.0 / 3.81 & 3.9 / 5.08 & 4.2 / 5.28 \\
Balance & VAR & 0.25 & 12.6 & 11.8 / 0.16 & 11.4 / 0.30 & 11.1 / 0.27 & 12.1 / 0.33 \\
Balance & VAR & 0.50 & 12.6 & 11.0 / 0.31 & 10.4 / 0.58 & 10.0 / 0.50 & 11.5 / 0.60 \\
Balance & VAR & 1.00 & 12.6 & 9.7 / 0.56 & 8.9 / 1.06 & 8.4 / 0.93 & 9.2 / 1.04 \\
Attention & VAR & 0.25 & 12.5 & 9.4 / 0.62 & 8.5 / 1.18 & 9.7 / 1.16 & 9.8 / 1.15 \\
Attention & VAR & 0.50 & 12.5 & 7.6 / 0.97 & 7.0 / 1.81 & 9.0 / 1.73 & 9.7 / 1.69 \\
Attention & VAR & 1.00 & 12.5 & 5.2 / 1.45 & 5.8 / 2.49 & 8.6 / 2.41 & 9.6 / 2.26 \\


==> tables/app_timescale.tex <==
Speaking & 1 & 0.279 & 0.293 & 0.715 & 0.010 & 0.014 & 0.782 & -0.063 & -0.081 \\
Speaking & 2 & 0.287 & 0.309 & 0.767 & 0.034 & 0.034 & 0.326 & -0.066 & -0.092 \\
Speaking & 4 & 0.270 & 0.288 & 0.727 & 0.093 & 0.087 & 0.220 & -0.069 & -0.101 \\
Speaking & 8 & 0.298 & 0.295 & 0.624 & 0.185 & 0.185 & 0.473 & -0.052 & -0.084 \\
Proximity & 1 & 0.127 & 0.135 & 0.480 & 0.021 & 0.016 & 0.063 & +0.030 & -0.038 \\
Proximity & 2 & 0.134 & 0.146 & 0.564 & 0.036 & 0.035 & 0.379 & +0.033 & -0.037 \\
Proximity & 4 & 0.131 & 0.140 & 0.566 & 0.061 & 0.072 & 0.875 & +0.039 & -0.039 \\
Proximity & 8 & 0.152 & 0.170 & 0.681 & 0.133 & 0.156 & 0.872 & +0.067 & -0.005 \\
Attention & 1 & 0.438 & 0.484 & 0.870 & 0.088 & 0.088 & 0.627 & -0.065 & -0.081 \\
Attention & 2 & 0.418 & 0.468 & 0.906 & 0.102 & 0.142 & 0.956 & -0.077 & -0.099 \\
Attention & 4 & 0.385 & 0.423 & 0.886 & 0.244 & 0.224 & 0.264 & -0.074 & -0.106 \\
Attention & 8 & 0.374 & 0.433 & 0.977 & 0.327 & 0.338 & 0.443 & -0.050 & -0.094 \\


==> tables/baselines.tex <==
\rowcolor{ours}ANCHOR (ours) & $52$ & 0.758 & \textbf{1.082} & 0.705 & \textbf{1.002} & 30\% \\
ANCHOR + observer & $56$ & 0.759 & \textbf{1.082} & 0.707 & 1.004 & 30\% \\
Attractor only & $21$ & 0.848 & 1.099 & 0.775 & 1.009 & 30\% \\
\midrule
Persistence & $0$ & 1.049 & 1.627 & 0.913 & 1.416 & \textbf{31\%} \\
Recent average & $0$ & 0.927 & 1.330 & 0.807 & 1.206 & \textbf{31\%} \\
Session mean & $0$ & 0.971 & 1.229 & 1.030 & 1.357 & 30\% \\
\midrule
VAR(2) & $820$ & 0.899 & 1.258 & 0.850 & 1.184 & 18\% \\
VAR(2) + aug. & $820$ & 0.826 & 1.242 & 0.780 & 1.170 & 15\% \\
Direct ridge & $43{,}840$ & 0.993 & 1.281 & 0.902 & 1.195 & 16\% \\
Ridge + aug. & $43{,}840$ & \textbf{0.754} & 1.110 & \textbf{0.703} & 1.044 & 27\% \\
MLP & $14{,}944$ & 1.084 & 1.291 & 1.073 & 1.340 & 17\% \\
MLP + aug. & $14{,}944$ & 1.057 & 1.258 & 1.004 & 1.253 & 18\% \\


==> tables/horizon.tex <==
1 & 16 & 0.50 & 1.20 & 58\% & 17/17 & 2e-5 & 2e-4 & 0.48 & 1.16 & 58\% & 17/17 & 2e-5 & 2e-4 \\
2 & 32 & 0.85 & 1.22 & 30\% & 17/17 & 2e-5 & 2e-4 & 0.78 & 1.17 & 33\% & 15/17 & 8e-5 & 0.001 \\
3 & 48 & 0.92 & 1.24 & 25\% & 16/17 & 1e-4 & 0.001 & 0.85 & 1.18 & 28\% & 15/17 & 2e-4 & 0.003 \\
4 & 64 & 0.97 & 1.25 & 22\% & 16/17 & 1e-4 & 0.001 & 0.91 & 1.20 & 24\% & 15/17 & 7e-4 & 0.009 \\
5 & 80 & 1.01 & 1.27 & 20\% & 14/17 & 4e-4 & 0.005 & 0.94 & 1.21 & 22\% & 13/17 & 0.002 & 0.025 \\
6 & 96 & 1.04 & 1.28 & 19\% & 13/17 & 0.003 & 0.028 & 0.97 & 1.22 & 21\% & 13/17 & 0.005 & 0.051 \\
7 & 112 & 1.07 & 1.30 & 18\% & 12/17 & 0.008 & 0.079 & 0.98 & 1.24 & 21\% & 12/17 & 0.007 & 0.067 \\
8 & 128 & 1.10 & 1.32 & 17\% & 12/17 & 0.017 & 0.157 & 1.01 & 1.26 & 20\% & 12/17 & 0.031 & 0.275 \\
10 & 160 & 1.15 & 1.38 & 16\% & 12/17 & 0.064 & 0.447 & 1.05 & 1.30 & 19\% & 10/17 & 0.132 & 1.000 \\
12 & 192 & 1.24 & 1.44 & 14\% & 11/17 & 0.174 & 0.871 & 1.13 & 1.35 & 17\% & 11/17 & 0.263 & 1.000 \\
16 & 256 & 1.30 & 1.51 & 14\% & 10/16 & 0.274 & 0.899 & 1.25 & 1.44 & 13\% & 6/16 & 0.900 & 1.000 \\


==> tables/intervention.tex <==
Balance & ANCHOR & 13.3 & 11.4 (4.7) & 11.4 (3.8) & 10.8 (5.1) & 12.1 (1.8) \\
Attention & ANCHOR & 11.5 & 5.7 (4.7) & 5.6 (2.3) & 5.3 (1.9) & 5.6 (1.7) \\
Balance & VAR & 12.6 & 11.0 (4.7) & 10.4 (3.4) & 10.0 (4.8) & 11.5 (1.7) \\
Attention & VAR & 12.5 & 7.6 (4.7) & 7.0 (2.8) & 9.0 (1.9) & 9.7 (1.5) \\


==> tables/principles.tex <==
\rowcolor{ours}P1 Equilibrium anchored on three sources & $q^\star$ from recent behaviour only & +19.3\% (17/17, 2e-5) & +16.5\% (14/17, 0.004) & \textbf{supported} \\
\rowcolor{ours}P1 Equilibrium anchored on three sources & $q^\star$ from session history only & +3.4\% (14/17, 0.035) & +9.7\% (14/17, 0.020) & \textbf{supported} \\
\rowcolor{ours}P2 Deviations relax back (16--48\,s) & attractor only, no dynamics & +11.3\% (17/17, 2e-5) & +8.5\% (15/17, 5e-4) & \textbf{supported} \\
\rowcolor{ours}P3 Team states emerge (speaking balance) & computed from dyadic forecast & -- & +270.3\% (16/17, 3e-5) & \textbf{supported} \\
P4 Phase-dependent dissipation & single phase & +0.1\% (9/17, 0.782) & -0.4\% (7/17, 0.611) & not significant \\
P5 Task progress steers the equilibrium & no progress port & +1.6\% (9/17, 0.487) & +2.2\% (9/17, 0.644) & not significant \\
Dominance and conflict add friction & no friction features & -0.0\% (8/17, 0.459) & -0.1\% (7/17, 0.431) & not significant \\
Inertia (second order) & momentum added & +0.2\% (11/17, 0.487) & +0.2\% (5/17, 0.579) & not significant \\
\rowcolor{ours}Team topology ties the matrices & unconstrained matrices & +14.4\% (16/17, 4e-4) & +9.7\% (17/17, 2e-5) & \textbf{supported} \\


==> tables/robustness.tex <==
Noise $\sigma=0.05$ & 1.14 & 1.13 & 1.13 & 1.21 & 1.05 & 1.05 & 1.31 & 1.18 \\
Noise $\sigma=0.1$ & 1.47 & 1.47 & 1.17 & 1.29 & 1.11 & 1.11 & 1.38 & 1.20 \\
Noise $\sigma=0.2$ & 2.99 & 2.97 & 1.29 & 1.46 & 1.14 & 1.14 & 1.38 & 1.23 \\
Dropout $p=0.1$ & 1.01 & 1.01 & 1.12 & 1.16 & 1.01 & 1.01 & 1.12 & 1.16 \\
Dropout $p=0.3$ & 1.03 & 1.03 & 1.13 & 1.17 & 1.04 & 1.03 & 1.13 & 1.17 \\
Dropout $p=0.5$ & 1.04 & 1.04 & 1.14 & 1.17 & 1.06 & 1.04 & 1.15 & 1.18 \\


==> tables/sensitivity.tex <==
15th & 0.75 / 0.76 & 0.77 / 0.77 & 0.65 / 0.69 & 5/12 & 3.9$\times$ \\
25th (main) & 0.85 / 0.85 & 0.76 / 0.76 & 0.66 / 0.68 & 8/12 & 2.2$\times$ \\
35th & 0.75 / 0.77 & 0.77 / 0.79 & 0.66 / 0.69 & 8/12 & 1.4$\times$ \\


==> tables/structure.tex <==
Speaking (member) & 0.44 & 0.19 & 0.37 & -0.058 & 26 & 37 \\
Attention (dyad) & 0.18 & 0.81 & 0.01 & -0.073 & 17 & 28 \\
Proximity (dyad) & 0.10 & 0.41 & 0.50 & -0.066 & 28 & 55 \\
Team speaking level & 0.34 & 0.13 & 0.53 & -0.042 & 38 & 32 \\
Team attention density & 0.35 & 0.58 & 0.07 & -0.060 & 22 & 43 \\
Team proximity density & 0.19 & 0.46 & 0.35 & -0.111 & 15 & 78 \\
Team speaking balance & 0.43 & 0.02 & 0.56 & -0.254 & 12 & 22 \\


==> tables/team.tex <==
ANCHOR (ours) & 0.86 & 1.19 & 1.13 & 0.82 \\
Attractor only & 0.88 & 1.20 & 1.14 & 0.82 \\
Persistence & 1.22 & 1.61 & 1.58 & 1.25 \\
Recent average & 1.07 & 1.38 & 1.35 & 1.02 \\
VAR(2) + aug. & 0.97 & 1.61 & 1.25 & 0.86 \\
MLP + aug. & 1.11 & 1.61 & 1.26 & 1.04 \\


==> tables/warning.tex <==
\rowcolor{ours}ANCHOR (ours) & \textbf{0.85} & \textbf{74\%} & 31 & \textbf{0.76} & 57\% & 35 & 0.66 & 34\% & 29 \\
Attractor only & \textbf{0.85} & 73\% & 31 & \textbf{0.76} & 56\% & 35 & 0.62 & 28\% & 31 \\
Recent average & 0.83 & 68\% & 32 & \textbf{0.76} & \textbf{58\%} & 37 & 0.63 & 26\% & 32 \\
VAR(2) + aug. & 0.80 & 64\% & 30 & 0.69 & 43\% & 36 & 0.65 & 39\% & 28 \\
Ridge + aug. & 0.80 & 60\% & 31 & 0.71 & 42\% & 35 & \textbf{0.68} & \textbf{43\%} & 32 \\
MLP + aug. & 0.74 & 50\% & 31 & 0.72 & 51\% & 37 & 0.56 & 25\% & 33 \\


==> tables_v2/horizon.tex <==
1 & 16 & 0.50 & 1.20 & 58\% & 17/17 & 2e-5 & 2e-4 & 0.48 & 1.16 & 58\% & 17/17 & 2e-5 & 2e-4 \\
2 & 32 & 0.85 & 1.22 & 30\% & 17/17 & 2e-5 & 2e-4 & 0.78 & 1.17 & 33\% & 15/17 & 8e-5 & 0.001 \\
3 & 48 & 0.92 & 1.24 & 25\% & 16/17 & 1e-4 & 0.001 & 0.85 & 1.18 & 28\% & 15/17 & 2e-4 & 0.003 \\
4 & 64 & 0.97 & 1.25 & 22\% & 16/17 & 1e-4 & 0.001 & 0.91 & 1.20 & 24\% & 15/17 & 7e-4 & 0.009 \\
5 & 80 & 1.01 & 1.27 & 20\% & 14/17 & 4e-4 & 0.005 & 0.94 & 1.21 & 22\% & 13/17 & 0.002 & 0.025 \\
6 & 96 & 1.04 & 1.28 & 19\% & 13/17 & 0.003 & 0.028 & 0.97 & 1.22 & 21\% & 13/17 & 0.005 & 0.051 \\
7 & 112 & 1.07 & 1.30 & 18\% & 12/17 & 0.008 & 0.079 & 0.98 & 1.24 & 21\% & 12/17 & 0.007 & 0.067 \\
8 & 128 & 1.10 & 1.32 & 17\% & 12/17 & 0.017 & 0.157 & 1.01 & 1.26 & 20\% & 12/17 & 0.031 & 0.275 \\
10 & 160 & 1.15 & 1.38 & 16\% & 12/17 & 0.064 & 0.447 & 1.05 & 1.30 & 19\% & 10/17 & 0.132 & 1.000 \\
12 & 192 & 1.24 & 1.44 & 14\% & 11/17 & 0.174 & 0.871 & 1.13 & 1.35 & 17\% & 11/17 & 0.263 & 1.000 \\
16 & 256 & 1.30 & 1.51 & 14\% & 10/16 & 0.274 & 0.899 & 1.25 & 1.44 & 13\% & 6/16 & 0.900 & 1.000 \\


==> tables_v2/principles.tex <==
\rowcolor{ours}P1 Resting point anchored on three sources & $q^\star$ from recent behaviour only & +19.3\% (17/17, 2e-5) & +16.5\% (14/17, 0.004) & \textbf{supported} \\
\rowcolor{ours}P1 Resting point anchored on three sources & $q^\star$ from session history only & +3.4\% (14/17, 0.035) & +9.7\% (14/17, 0.020) & \textbf{supported} \\
\rowcolor{ours}P2 Deviations relax back (16--48\,s) & attractor only, no dynamics & +11.3\% (17/17, 2e-5) & +8.5\% (15/17, 5e-4) & \textbf{supported} \\
\rowcolor{ours}P3 Team states emerge (speaking balance) & computed from member forecast & -- & +270.3\% (16/17, 3e-5) & \textbf{supported} \\
P4 Phase-dependent regulation & single phase & +0.1\% (9/17, 0.782) & -0.4\% (7/17, 0.611) & not significant \\
P5 Task progress moves the resting point & no progress port & +1.6\% (9/17, 0.487) & +2.2\% (9/17, 0.644) & not significant \\
Dominance and conflict add damping & no sensed damping & -0.0\% (8/17, 0.459) & -0.1\% (7/17, 0.431) & not significant \\
Inertia (second order) & momentum added & +0.2\% (11/17, 0.487) & +0.2\% (5/17, 0.579) & not significant \\
\rowcolor{ours}Team structure ties the matrices & unconstrained matrices & +14.4\% (16/17, 4e-4) & +9.7\% (17/17, 2e-5) & \textbf{supported} \\


==> tables_v2/principles_old.tex <==
\rowcolor{ours}P1 Resting point anchored on three sources & $q^\star$ from recent behaviour only & +19.3\% (17/17, 2e-5) & +16.5\% (14/17, 0.004) & \textbf{supported} \\
\rowcolor{ours}P1 Resting point anchored on three sources & $q^\star$ from session history only & +3.4\% (14/17, 0.035) & +9.7\% (14/17, 0.020) & \textbf{supported} \\
\rowcolor{ours}P2 Deviations relax back (16--48\,s) & attractor only, no dynamics & +11.3\% (17/17, 2e-5) & +8.5\% (15/17, 5e-4) & \textbf{supported} \\
\rowcolor{ours}P3 Team states emerge (speaking balance) & computed from member forecast & -- & +270.3\% (16/17, 3e-5) & \textbf{supported} \\
P4 Phase-dependent regulation & single phase & +0.1\% (9/17, 0.782) & -0.4\% (7/17, 0.611) & not significant \\
P5 Task progress moves the resting point & no progress port & +1.6\% (9/17, 0.487) & +2.2\% (9/17, 0.644) & not significant \\
Dominance and conflict add damping & no sensed damping & -0.0\% (8/17, 0.459) & -0.1\% (7/17, 0.431) & not significant \\
Inertia (second order) & momentum added & +0.2\% (11/17, 0.487) & +0.2\% (5/17, 0.579) & not significant \\
\rowcolor{ours}Team structure ties the matrices & unconstrained matrices & +14.4\% (16/17, 4e-4) & +9.7\% (17/17, 2e-5) & \textbf{supported} \\

